Competitive Distribution Estimation

Estimating an unknown distribution from its samples is a fundamental problem in statistics. The common, min-max, formulation of this goal considers the performance of the best estimator over all distributions in a class. It shows that with $n$ samples, distributions over $k$ symbols can be learned to a KL divergence that decreases to zero with the sample size $n$, but grows unboundedly with the alphabet size $k$. Min-max performance can be viewed as regret relative to an oracle that knows the underlying distribution. We consider two natural and modest limits on the oracle's power. One where it knows the underlying distribution only up to symbol permutations, and the other where it knows the exact distribution but is restricted to use natural estimators that assign the same probability to symbols that appeared equally many times in the sample. We show that in both cases the competitive regret reduces to $\min(k/n,\tilde{\mathcal{O}}(1/\sqrt n))$, a quantity upper bounded uniformly for every alphabet size. This shows that distributions can be estimated nearly as well as when they are essentially known in advance, and nearly as well as when they are completely known in advance but need to be estimated via a natural estimator. We also provide an estimator that runs in linear time and incurs competitive regret of $\tilde{\mathcal{O}}(\min(k/n,1/\sqrt n))$, and show that for natural estimators this competitive regret is inevitable. We also demonstrate the effectiveness of competitive estimators using simulations.

==> ignored.tex <==
\ignore{
where the expectation is over the $\dist$ for generating sequences $\seq$
and the randomization of the estimator $\est$. A related notion of
accuracy are high-probability results which require for most sequences
$\KL{\dist}{\est}$ to be small, \ie $\KL{\dist}{\est} \leq \cdot$,
with probability $\geq 1-\epsilon$, where the probability is over
$\dist$ for generating sequences $\seq$ and the randomization of the
estimator $\est$. To the best of our knowledge, most of the results
which hold in expectation also hold in high probability terms with an
additional $\log \frac{1}{\epsilon}$ term. To simplify the analysis,
we focus on the expectation.
}
\ignore{
The first question that arises in probability estimation would be to ask what is the best estimator for a given distribution $p$. More specifically, find $\est$ such that
\[
\min_{\est}  \EE [\KL{\dist}{\est}].
\]
The answer to this question is trivial with $\ests{x} = \ps{x}, \forall x$, irrespective of the observed sequence. For this estimator 
\[
  \EE [\KL{\dist}{\est}] = 0.
\]
This is the best possible estimator as $\KL{\dist}{\est}$ is always non-negative.
}
%To overcome these trivial estimators, we need that the estimators
%  work well for at least two distributions or in general we need the
%  estima%tor to work well for a class of distributions $\cP$.  obtain
%  meaningful answers, two approaches are popularly used Bayesian, or
%  Frequentist. We first describe the Bayesian approach.  The bayesian
%  approach, assumes a prior on the set of candidate distributions
%  $\cP$ the prior denoted by $\prior$, \ie $\prior$ associates a
%  probability $\prior(\dist)$ for every distribution in $\cP$ such
%  that \[ \sum_{\dist \in \cP} \prior(\dist) = 1.  \] Thus the
%  Bayesian estimators asks for the best estimator for this class
%  according to the prior.  \[ \min_{\est} \EE_\prior \EE
%  [\KL{\dist}{\est}].  \] It is well known that the best estimator is
%  the one that gives each $\sym$, the posterior probability after
%  observing $\seq$.  \[ \ests{\sym} = \frac{\sum_{\dist}
%  \prior(\dist) \ps{\seq}\ps{\sym}}{\sum_{\dist'} \prior(\dist')
%  \ps{\seq}'} \] Note that the above answer holds for any class $\cP$
%  and any prior $\prior$. The above analysis motivated several
%  add-$\beta$ estimators.  Let $\Deltak$ denote the class of
%  distributions over the set $\{1,2,\ldots k\}$, then the popular
%  prior on this class of distributions is the% Dirchlet prior $\beta$
%  is \[ \pi(dist) \propto \prod_{\sym \in \cX}
%  \ps{\sym}^{\beta-1}.  \] It can be showed that the best estimator
%  under Direchlet prior $\beta$ is \[ \ests{\sym} =
%  \frac{\mul{\sym}+\beta}{\sam+\alp \beta}, \] thus motivating add
%  $\beta$ estimators.  To overcome this triviality, is to design an
%  estimator that works well for for every $\dist \in \cP$,\ie

%A \emph{partition} $\PP$ of a set $\cP$ is a collection of disjoint
%subsets of $\cP$ whose union is $\cP$. 
%For the rest of this result we set $\cP = \Deltak$.

%A natural question is to ask if there is an estimator that does the
%best it can for every distribution in the class? To formalize this
%question, we need few definitions.

%\cP_i \in \PP$, the best error possibilities $\errorn{\cP_i}$, is
%there an estimator that uniformly achieves this?



==> notation.tex <==
\section{Notation}


We use $\sam$ to denote the number of samples 

